(Noisy) Gap Cycle Counting Strikes Back: Random Order Streaming Lower Bounds for Connected Components and Beyond

We continue the study of the communication complexity of gap cycle counting problems. These problems have been introduced by Verbin and Yu [SODA 2011] and have found numerous applications in proving streaming lower bounds. In the noisy gap cycle counting problem (NGC), there is a small integer $k \geq 1$ and an $n$-vertex graph consisted of vertex-disjoint union of either $k$-cycles or $2k$-cycles, plus $O(n/k)$ disjoint paths of length $k-1$ in both cases (``noise''). The edges of this graph are partitioned between Alice and Bob whose goal is to decide which case the graph belongs to with minimal communication from Alice to Bob. We study the robust communication complexity -- `a la Chakrabarti, Cormode, and McGregor [STOC 2008] -- of NGC, namely, when edges are partitioned randomly between the players. This is in contrast to all prior work on gap cycle counting problems in adversarial partitions. While NGC can be solved trivially with zero communication when $k < \log{n}$, we prove that when $k$ is a constant factor larger than $\log{n}$, the robust (one-way) communication complexity of NGC is $\Omega(n)$ bits. As a corollary of this result, we can prove several new graph streaming lower bounds for random order streams. In particular, we show that any streaming algorithm that for every $\varepsilon > 0$ estimates the number of connected components of a graph presented in a random order stream to within an $\varepsilon \cdot n$ additive factor requires $2^{\Omega(1/\varepsilon)}$ space, settling a conjecture of Peng and Sohler [SODA 2018]. We further discuss new implications of our lower bounds to other problems such as estimating size of maximum matchings and independent sets on planar graphs, random walks, as well as to stochastic streams.

==> kpeople.tex <==



\section{Batched Random Order Lower Bounds for $\NGC_{n,k}$}

In this section, we will prove lower bounds against a batched random order streaming model for $\NGC_{n,k}$ when $k = \Theta\paren{\frac{\log n}{\log \log n}}$, by considering an $\ell$ player one-way communication model with edges distributed uniformly at random between them. Then, we show that this leads to a stronger lower bound $(1/\eps)^{\Omega(1/\eps)}$ for estimation of number of connected components up to an additive $\eps \cdot n$ factor in this edge arrival model. 

\subsection{Setting Up}

We will start by adapting the definitions of our communication problems to players $\people$ instead of just Alice and Bob. 

\begin{definition}\label{def:ngcl}
	The \textbf{Noisy Gap Cycle Counting $\NGCl_{n,k}$} communication problem is as follows. We have a graph $G = (V,E)$ on $n $ vertices such that $G$ either contains,
	\begin{itemize}
		\item $(n/4k)$ vertex-disjoint cycles of length $2k$, or
		\item $(n/2k)$ vertex-disjoint cycles of length $k$.
	\end{itemize}
	
	The edges of $G$ are split into $\card{E}/2$ batches $(\batch{1}, \batch{2}, \ldots,\batch{\card{E}/2})$ of size two each. Let $\batch{j} = (e^j_1, e^j_2)$ be the two edges in partition $\batch{j}$ for $j \in [\card{E}/2]$. 
	
	There are $\ell$ players $\people$. For each $i \in [\ell]$, $\person{i}$ is given as input $G_i = (V, E_i)$ such that $E = \cup_{i \in [\ell]} E_i$. Both edges in each partition $\batch{j}$, $j \in [\card{E}/2]$ is added to $E_{i}$ where $i$ is picked uniformly at random from $[\ell]$.
	
	$\person{i}$ can send messages only to $\person{i + 1}$ for $i \in [\ell-1]$, and $\person{\ell}$ has to distinguish whether there are cycles of length $k$ or $2k$ with probability at least 2/3 for \emph{any} possible partitioning of the edges. 
\end{definition}

Next, we show that $\NGCl_{n,k}$ reduces to estimating the number of connected components in batched random order streams.

\begin{lemma}\label{lem:cctongc-l}
	If there exists a streaming algorithm $\alg$ for connectivity in batched random order edge arrival which uses $s$-space with an additive approximation $\eps \cdot n$ with $\eps  < 1/8k$ with probability of success at least 2/3, then there exists a protocol for $\NGCl_{n,k}$ where the message length is at most $s$. 
\end{lemma}

\begin{proof}
	There is a difference of $n/4k$ in the number of connected components in either cases of $\NGCl_{n,k}$. 
	The streaming algorithm $\alg$ finds the number of connected components to within an additive factor of $\eps\cdot n < n/8k$ when the batches arrive in random order. On the input graph $G$, the players can simulate the algorithm $\alg$ as follows. Starting from $\person{1}$,
	\begin{enumerate}
		\item Player $\person{i}$ picks a random permutation of the batches in $E_i$ , and runs algorithm $\alg$ on this ordering after all batches in $E_j$ for $j < i$ have been given to $\alg$. 
		\item Player $\person{i}$ then sends the state of algorithm $A$ using $s$-bits to $\person{i +1}$. 
	\end{enumerate} 
	This is a correct simulation of $\alg$ on the input graph of $\NGCl$ as the edges of $E$ arrive in batched random order. 
	
	If the total number of connected components from $\alg$ is at least $7n/8k$, then the graph consists only of cycles of length $k$. Otherwise the graph contains cycles of length $2k$. $\person{\ell}$ can distinguish the two cases from the number of connected components found by $\alg$ with probability of success at least 2/3. 	
\end{proof}

From \Cref{lem:cctongc-l}, it is clear that any lower bound on $\NGCl$ gives a corresponding lower bound for connectivity. 
We will move to describing the hard distribution for $\NGCl$ next. We need a few more definitions building on XOR-Matchings from \Cref{def:xor-matching} and Perm-Matchings from  \Cref{def:perm-matching} to do so. 

\begin{definition}\label{def:permxor}
	Given an $x \in \set{0,1}^{\ww}$ and a permutation $\sigma \in \mathcal{S}_{\ww}$, a graph $G \in \LG_{\ww,3}$ is a Perm-XOR-matching $\permxor{\sigma, x}$ if $G = \permmatch{\sigma} \conc \xormatch{x}$.  
\end{definition}

We combine multiple Perm-XOR-matchings along with a final Perm-matching for a specific permutation to get a Segment as follows.

\begin{definition}\label{def:segment}
	Given $X = (x^1, x^2, \ldots, x^t) \in \paren{\set{0,1}^{\ww}}^t$ and $\Sigma = (\sigma^1, \sigma^2, \ldots, \sigma^t) \in \paren{\mathcal{S}_{\ww}}^t$, $G\in \LG_{\ww, 2t+2}$ is a segment graph $\segment{X, \Sigma}$ if, 
	\begin{align*}
		G =  \permxor{\sigma^1, x^1} & \conc \permxor{\sigma^1_{-1}  \circ \sigma^2, x^2} \conc \permmatch{\sigma^2_{-1}  \circ \sigma^3, x^3} \\
		&\conc\ldots \conc \permxor{\sigma^{t-1}_{-1} \circ \sigma^t, x^t} \conc \permmatch{\sigma^t_{-1}}. 
	\end{align*}
	We define $z_G(j) = \bigoplus_{i \in [t]} x^i_{\sigma^i(j)}$. 
\end{definition}

\begin{claim}\label{clm:segment}
	In any graph $G = \segment{X, \Sigma} \in \LG_{\ww, 2t+2}$, for each $j \in [\ww]$,
	\begin{enumerate}[label=$(\roman*)$]
		\item $P_G(j) = j$.
		\item Paths $a^1_j \rightsquigarrow b^{2t+2}_j$ and $b^1_j \rightsquigarrow a^{2t+2}_j$ exist if $z_G(j) = 1$, else $a^1_j \rightsquigarrow a^{2t+2}_j$ and $b^1_j \rightsquigarrow b^{2t+2}_j$.
	\end{enumerate}
\end{claim}
\begin{proof}
	For any graph $G' = \permxor{\sigma, x}$, we know $P_{G'}(j) = \sigma(j)$. By \Cref{obs:concatenate-2},
	\begin{align*}
		P_{G}(j) = \sigma^t_{-1} ( \sigma^t ( \sigma^{t-1}_{-1} ( \sigma^{t-1} (\ldots ( \sigma^2 \circ \sigma^1_{-1} \circ \sigma^1(j)))) \ldots ) = j. 
	\end{align*}
Let $G_i = \permxor{\sigma^1, x^1} \conc \ldots \conc \permmatch{\sigma^{i-1}_{-1}  \circ \sigma^i, x^i}$. We use induction to prove part $(ii)$.
	We analyze the two possible cases for the value taken by $z_{G_i}(j)$ as follows.
\begin{itemize}
	\item If $z_{G_{i-1}}(j) = x^i_{\sigma^i(j)} $, then $z_{G_i}(j) = 0$. If $z_{G_{i-1}}(j) = x^i_{\sigma^i(j)} = 0$, we have paths from $a^1_j \rightsquigarrow a^{2i+1}_j \rightsquigarrow a^{2(i+1)+1}_j$ and $b^1_j \rightsquigarrow b^{2i+1}_j \rightsquigarrow  b^{2(i+1)+1}_j$.  If $z_{G_{i-1}}(j) = x^i_{\sigma^i(j)} = 1$, then we have paths from $a^1_j \rightsquigarrow b^{2i+1}_j \rightsquigarrow a^{2(i+1)+1}_j$ and $b^1_j \rightsquigarrow a^{2i+1}_j \rightsquigarrow  b^{2(i+1)+1}_j$. 
	\item If $z_{G_i}(j) = 1$, then either $z_{G_{i-1}}(j) = 0, x^i_{\sigma^i(j)} = 1$, where we have with paths from $a^1_j \rightsquigarrow a^{2i+1}_j \rightsquigarrow b^{2(i+1)+1}_j$ and $b^1_j \rightsquigarrow b^{2i+1}_j \rightsquigarrow  a^{2(i+1)+1}_j$,
	or $z_{G_{i-1}}(j) = 1, x^i_{\sigma^i(j)} = 0$, with paths from $a^1_j \rightsquigarrow b^{2i+1}_j \rightsquigarrow b^{2(i+1)+1}_j$ and $b^1_j \rightsquigarrow a^{2i+1}_j \rightsquigarrow  a^{2(i+1)+1}_j$. 
\end{itemize}
\end{proof}

We can combine multiple segments to get a larger group layered graph.

\begin{definition}\label{def:multisegment}
	Given $X = (X_1, X_2, \ldots, X_s)$ and $\Sigma = (\Sigma_1, \ldots, \Sigma_s)$ with $X_i = (x^{i,1}, x^{i,2}, \ldots, x^{i,t}) \in \paren{\set{0,1}^{\ww}}^t$ and $\Sigma_i = (\sigma^{i,1}, \sigma^{i,2}, \ldots, \sigma^{i,t}) \in \paren{\mathcal{S}_{\ww}}^t$ for $i \in[s]$, $G\in \LG_{\ww, (2t+1)s+1}$ is a multi-segment graph $\multisegment{X, \Sigma}$ if, 
	\begin{align*}
		G =  \segment{X_1, \Sigma_1} \conc \segment{X_2, \Sigma_2} \conc \ldots \conc \segment{X_s, \Sigma_s}. 
	\end{align*}
	We define $z_G(j) = \bigoplus_{i \in [s]} \bigoplus_{i' \in [t]} x^{i,i'}_{\sigma^{i,i'}(j)}$.  We denote by $S_i$ segment $i$ based on $X_i, \Sigma_i$ for $i \in [s]$. 
\end{definition}

\begin{claim}\label{clm:multisegment}
	In any graph $G = \multisegment{X, \Sigma} \in \LG_{\ww, d}$, for each $j \in [w]$,  
	\begin{enumerate}[label=$(\roman*)$]
		\item $P_G(j) = j$.
		\item Paths $a^1_j \rightsquigarrow b^{d}_j$ and $b^1_j \rightsquigarrow a^{d}_j$ exist if $z_G(j) = 1$, else $a^1_j \rightsquigarrow a^{d}_j$ and $b^1_j \rightsquigarrow b^{d}_j$.
	\end{enumerate}
\end{claim}
\begin{proof}
	In each segment we know $P_{S_i}(j) = j$. Hence in the larger graph $G$ we have $P_G(j) = j$ by \Cref{obs:concatenate-2}. 
	Part $(ii)$ follows by an induction on $i$ as we have seen in proofs of \Cref{clm:segment,obs:multi-block}.
\end{proof}

\subsection{Hard Distribution}

Our hard distribution is now a multi-segment graph with auxiliary edges. 

\begin{tbox}
	\textbf{A hard distribution $\distNGCl$ for $\NGC_{n,k}$} (when $k=(2t+1)s + 1$ for $t, s \geq 1$ and $n=4k \cdot m$ for $m \geq 1$).
	\begin{enumerate}[label=$(\roman*)$]
		\item Sample $ \theta $ uniformly at random from $\set{0,1}$.
		\item Sample $X \in \paren{\set{0,1}^{2m}}^{st}$ and $\Sigma  \in \paren{\mathcal{S}_{2m}}^{st}$ uniformly at random conditioned on the event that for all $j \in [m]$:
		\[
		\bigoplus_{i \in [s]} \bigoplus_{i' \in [t]} x^{i,i'}_{\sigma^{i,i'}(j)} = \theta.
		\]
		\item Let $G = \multisegment{X,\Sigma} \in \LG_{2m,k}$ plus the \emph{auxiliary edges} $(a^{k}_j,a^1_j)$ and $(b^k_j,b^1_j)$ for $j \in [m]$. 
		\item The edges of $G$ are partitioned into $\card{E}/2$ batches where both the edges associated with $x^{i, i'}_j$ and $\sigma^{i,i'}(j)$ are put in the same batch. 
	\end{enumerate}
\end{tbox}

\begin{lemma}\label{lem:distNGChidden}
	For any graph $G \sim \distNGCl$ for $\NGC_{n,k}$: 
	\begin{enumerate}[label=$(\roman*)$]
		\item if $\theta = 0$, $G$ has $(n/2k)$ vertex-disjoint cycles of length $k$; 
		\item if $\theta = 1$, $G$ has $(n/4k)$ vertex-disjoint cycles of length $2k$. 
	\end{enumerate}
	In either case, $G$ additionally has $(n/2k)$ vertex-disjoint paths of length $k-1$. 
\end{lemma}

\begin{proof}
\end{proof}

\begin{problem}[\textbf{(Distributional) Hidden-XOR Problem} (\DHXORl)]\label{def:dhxor-l}
	In $\DHXORl_{\ww, s, t}$, we have a graph $G = \multisegment{X,\Sigma} \in \LG_{\ww,(2t+1)s+1}$ for $X \in \paren{\set{0,1}^{\ww}}^{st}$ and $\Sigma \in \paren{\mathcal{S}_{\ww}}^{st}$ chosen independently and uniformly at random. 
	The edges in $G$ are partitioned into batches of size two each such that both the edges based on each value $x^{i,i'}_j$ and each part of permutation $\sigma^{i,i'}(j)$ are in the same batch.
	The goal is for $\person{\ell}$ to output $z_G(1)$ in this graph when the batches are \emph{randomly} partitioned between $\people$ and $\person{i}$ can send messages to $\person{i + 1}$ for $i \in [\ell-1]$ only. 
\end{problem}

\begin{lemma}\label{lem:main-ngc-l}
	For any sufficiently large $n \geq 1$, $k = (2t+1)s+1$ for some $t,s \geq 1$ and $\ww = (n/4k)+1$, 
	\[
	\oDD{\distNGCl}{1/3}(\NGCl_{n,k}) \geq \oDD{\distDHXl}{\frac{1}{2}-\frac{1}{6\ww}}(\DHXORl_{\ww, s, t}), 
	\] 
	where $\distDHXl$ is the implicit uniform distribution in the definition of $\DHXORl$. 
\end{lemma}

\begin{tbox}
	\textbf{Distribution} $\distHNGCl(h)$\textbf{.} Sample $X   \in  \paren{\set{0,1}^{2m}}^{st}$, $\Sigma = \in \paren{\mathcal{S}_{2m}}^{st}$  independently and uniformly at random conditioned on
	\begin{align*}
		z_G(j) = \bigoplus_{i \in [s]} \bigoplus_{i' \in [t]} x^{i,i'}_{\sigma^{i,i'}(j)}= 
		\begin{cases}
			0 &\textnormal{ if $j \leq h$,} \\
			1 & \textnormal{  otherwise},
		\end{cases}
	\end{align*}
for each $j \in [m]$. 
\end{tbox}

\begin{lemma}\label{lem:hybridindexl}
	There exists an index $1 \leq \istar \leq m$ such that protocol $\Pi$ can distinguish the samples from $\distHNGCl(\istar-1)$ and $\distHNGCl(\istar)$ with probability at least $\frac12 + \frac1{6m}$. 
\end{lemma}

\begin{proof}
\end{proof}

\begin{Algorithm}\label{alg:samplngch-l}
	A protocol for $\DHXORl_{\ww, s, t}$ using protocol $\Pi$ for $\NGCl_{n,k}$ with $\ww = \frac{n}{4k}+1, k = (2t+1)s+1$. 
	
	\smallskip
	
	\textbf{Input:} An instance of $\DHXOR_{\ww,t}$,  $G = \multisegment{Y, \Tau}$, $Y  \in \paren{\set{0,1}^{\ww}}^{st}$, and $\Tau  \in \paren{\mathcal{S}_{\ww}}^{st}$.  
	
	\smallskip
	
	\textbf{Output:} Answer to $\DHXOR_{\ww, t}$ on $G$, i.e., $z_G(1)$.
	\begin{enumerate}[label=$(\roman*)$]
		%	\item For $i \in [k]$, denote $V^i := [2\ww]$. 
		\item Sample $\Sigma_{[m]\setminus\set{\istar}} \coloneqq (\Sigma^1, \ldots, \Sigma^s) \in \paren{\mathcal{S}_{2m}^{[m]\setminus\set{\istar}}}^{st}$ uniformly at random.
		\item Let $I^i_{\circ} = \set{\sigma^i(j) \mid j \in \paren{[m]\setminus \set{\istar}}}$ for $i \in [t]$, that is, $I^i_{\circ}$ is the set of indices that have a non-$\star$ pre-image under permutation $\sigma^i$. The set $I^i_{\circ}$ has $m-1$ elements for all $i \in [st]$. 
		\item Sample $X_{[m]\setminus\set{\istar}} = (x^{1,1}, x^{1,2}, \ldots, x^{1,t}, x^{2,1}, \ldots, x^{s,t}) \in \paren{\cU_{2m}^{I^1_{\circ}} \times \cU_{2m}^{I^2_{\circ}} \times \ldots \cU_{2m}^{I^{st}_{\circ}}}$ uniformly at random conditioned on the event that,
		\begin{align*}
			\bigoplus_{i \in [s]} \bigoplus_{i' \in [t]} x^{i,i'}_{\sigma^{i,i'}(j)}= 
			\begin{cases}
				0 &\textnormal{ if $1 \leq j \leq \istar-1$,} \\
				1 & \textnormal{  if $\istar+1 \leq j \leq m$}.
			\end{cases}
		\end{align*}
		\item Lexicographically map indices $[m+1]$ to $[2m] \setminus I^i_{\circ}$ for each $i \in [st]$. This is possible since $\card{[2m] \setminus I^i_{\circ}} = m+1 = \ww$. Denote this mapping by $f_i : [m+1] \rightarrow [2m] \setminus I^i_{\circ}$. 
		\item Update the positions with $\star$ value in $X_{[m]\setminus\set{\istar}}$ and $\Sigma_{[m]\setminus\set{\istar}}$ to get $X$ and $\Sigma$ respectively as follows. For each $i \in [t]$,
		\begin{align*}
			\sigma^i(j) = \begin{cases}
				f_i(\ttau^i(1)) &\textnormal{if $j = \istar$} \\
				f_i(\ttau^i(j-m+1)) &\textnormal{if $m < j \leq 2m$ }
			\end{cases}
			&& \textnormal{and} &&
			x^i_{f_i(j)} = y^i_{j} &\hspace{4mm} \textnormal{for $j \in [m+1]$.}
		\end{align*}
		\item Fix $G' = \multiblock{X, \Sigma}$. 
		\item Run protocol $\Pi$ on $G'$ to identify whether $G' \sim \distHNGC(\istar-1)$ or $G' \sim \distHNGC(\istar)$; in the former case output $0$ and in the latter output $1$.
	\end{enumerate}
\end{Algorithm}


\subsection{Lower Bound for Distributional Hidden XOR}

In this section we prove a lower bound for the $\DHXORl_{\ww, s, t}$ problem when the number of layers $k = \Theta\paren{\frac{\log n}{\log \log n}}$.

\begin{definition}\label{def:active-segment}
	A segment $S_i = \segment{X_i, \Sigma_i}$ is said to be \textbf{active} if on the path from the starting group $g^{(2t+1)(i-1)+1} $ to $g^{(2t+1)i+1}_1$, there exists a group $g^{(2t+1)(i-1) + 2{\spi}}_{j}$, $\spi \in [t], j \in [\ww] $ such that the edges out of this group are sent to $\person{\beta}$ and the edges into this group are sent to $\person{\alpha}$ such that $\frac{\ell}s \cdot (i-1) +1 \leq \beta < \alpha \leq \frac{\ell}{s} \cdot i$.
\end{definition}

\begin{lemma}\label{lem:active-segment}
	For $t \geq 8s^2 \frac{\log w}{\log \log w}$, all segment $S_i$ for $i \in [s]$ are active with probability at least $1-\frac1{w^4}$. 
\end{lemma}

\begin{proof}
	The edges into and out of each group in all the segments of $G$ are sent to a person picked uniformly at random out of $\people$. 
	There are $\ell^2$ possible choices for how the edges into and out of group $g^{(2t+1)(i-1) + 2a}_{j}$ are distributed for $a \in [t]$ ($\ell$ choices for the edges into the group and $\ell$ choices for edges out of the group). 
	There are $\frac{\ell}{2s} \cdot \paren{\frac{\ell}{s}-1}$ choices for $\alpha, \beta$ to make segment $S_i$ active. Thus, for any $a \in [t]$, 
	\begin{align*}
		\prob{\textnormal{Group $g^{(2t+1)(i-1) + 2a}_{j}$ makes $S_i$ active}} &= \frac1{\ell^2} \cdot \frac{\ell}{2s} \cdot  \paren{\frac{\ell}{s}-1} \geq \frac1{4s^2}. 
	\end{align*}
Let $R_a$ be the indicator for whether the above event happens for $a \in [t]$. We want to prove that $R = \sum_{a \in t} R_a = 0$ happens with low probability. All the $R_a$s are independent by definition of $\DHXORl_{\ww, s, t}$. We know $\expect{R} \geq 2 \log \ww/\log \log \ww$. 
\begin{align*}
	\prob{\sum_{a \in t} R_a < 1} &\leq \paren{e^{1}}\paren{1-\frac1{4s^2}}^{8s^2  \cdot  \frac{\log w}{\log \log w}} \leq 
\end{align*}
\end{proof}

We will condition on all the segments being active for the rest of this section. 

\newcommand{\eventgood}{\event_{\texttt{good}}}
\newcommand{\eventact}{\event_{\texttt{act}}}

\paragraph{Notation.} 
Let the group which makes segment $S_i$ active be denoted by index $\spi(i) \in [t]$ for $i \in [s]$. Let the edges out of group $g^{(2t+1)(i-1) + 2\spi(i)}_{j}$ be sent to $\person{\alpha(i)}$ and the edges into the group be sent to $\person{\beta(i)}$. 

We call a group $g^{(2t+1)(i-1) + 2\spi(i)}_j$ a \textbf{good} group if the edges out of this group into the next layer are sent to $\person{\alpha(i)}$, and the edges into this group from the previous layer are sent to $\person{\beta(i)}$.  Let $\eventgood$ be used to denote the event that at least $\frac{\ww}{2\ell^2}$ groups are good for all segments $S_i$. Let $\eventact$ be used to denote the event that all the segments in $G$ are active. 

\begin{lemma}\label{lem:good-groups}
For any active segment $S_i$, if $\ell = O(1)$ and $s = O(1)$, event $\eventgood$ happens with probability at least $1-\frac1{\ww^5}$. 
\end{lemma}

\begin{proof}
	Let $R_j$ be the indicator variable for whether the edges out of group $g^{(2t+1)(i-1) + 2\spi(i)}_j$ are sent to $\person{\alpha}$, and the edges into this group are sent to $\person{\beta(i)}$.  Each $R_j = 1$ with probability $\frac1{\ell^2}$ and 0 otherwise indpendently. We want to lower bound the probability that $\sum_{j=1}^{\ww} R_j \geq \frac{\ww}{2\ell^2}$. As the $R_j$s are independent, we use Chernoff bound from \Cref{prop:chernoff} here. 
\begin{align*}
	\prob{R < \frac{\ww}{2\ell^2}} &= \prob{R < \paren{1-\frac12} \cdot \expect{R}} \\
	&\leq \exp\paren{\frac{-1}4 \cdot \frac{\ww}{2\ell^2} \cdot \frac13} \\
	&\leq \frac1{\ww^6}. 
\end{align*}
Using a union bound over all $s = O(1)$ segments, we prove the claim.
\end{proof}

We can condition on both $\eventact$ and $\eventgood$ happening for input graph instance $G$ while decreasing the probability of success only slightly. 

\begin{lemma}\label{lem:cond-act-good}
	Any protocol $\Pi$ solving $\DHXOR_{\ww, t}$ for $t \geq 8s^2 \frac{\log w}{\log \log w}$, $s = O(1)$ and $\ell = O(1)$ with probability at least $\frac12+ \frac1{6w}$, solves $\DHXOR_{\ww, t}$ even conditioned on events $\eventgood$ and $\eventact$ with probability at least $\frac12 + \frac1{8\ww} $ for sufficiently large $\ww$. 
\end{lemma}

\begin{proof}
		Let $\Pi(G)$ denote the output of protocol $\Pi$ on input graph $G$. For any input $G$,
	\begin{align*}
		\prob{\Pi(G) = z_G(1)} &\leq \prob{\neg \eventact \textnormal{ or }\neg \eventgood}+ \prob{\eventact, \eventgood} \cdot \prob{\Pi(G) = z_G(1) \mid  \eventact, \eventgood} \\
		&\leq \prob{\neg \eventact} +\prob{\neg \eventgood} + \prob{\Pi(G) = z_G(1) \mid  \eventact, \eventgood} \\
		&\leq \frac1{w^4} +  \prob{\neg \eventgood} + \prob{\Pi(G) = z_G(1) \mid \eventact, \eventgood} \tag{by \Cref{lem:active-segment}} \\
		&\leq \frac2{w^3} + \prob{\Pi(G) = z_G(1) \mid \eventA,\eventC}.  \tag{by \Cref{lem:good-groups}}
	\end{align*}
	Hence, for sufficiently large $w$, 
	\begin{align*}
		\prob{\Pi(G) = z_G(1) \mid \eventact,\eventgood} \geq \frac12 + \frac1{6w}-\frac2{w^3} \geq \frac12 + \frac1{8w}. \qedhere
	\end{align*}
\end{proof}

Next we 

\begin{lemma}\label{lem:cond-rest-l}
	In each segment
\end{lemma}



\clearpage


==> maxindset.tex <==

\section{Proof of \Cref{thm:indsetest}}\label{app:indsetprf}
\begin{proof}
	Any instance of $\NGC_{n,k}$ is a planar graph of degree two for any $n,k$ as it is just a collection of cycles and paths. 
	
	For any odd $k$, in an instance of $\NGC_{n,k}$, each path of length $k-1$ has an independent set of size at most  of $(k+1)/2$ vertices. If the instance contains cycles of length $2k$, each such cycle has an independent set with $k$ vertices. The size of the maximum independent set is $(n/4k) \cdot k + (n/2k) \cdot \paren{(k+1)/2}$. If the instance instead has cycles of length $k$, then each such cycle has an independent set of $(k-1)/2$ vertices, and the maximum independent set is of size $(n/2k) \cdot \paren{(k+1)/2} + (n/2k) \cdot (k-1)/2$. There is a difference of $(n/4k)$ in either case of $\NGC_{n,k}$. 
	
	Given a random order one pass streaming algorithm which gives a $(1+\eps)$ approximation of maximum independent set for $ \eps < \frac1{2k}$, if the $\NGC_{n,k}$ instance has cycles of length $2k$, then the algorithm outputs that an independent set of size at least $n(2k+1)/4k \cdot \frac1{1+\eps} > n(2k)/4k$. This is more than the size of the maximum independent set when the instance has cycles of length $k$. Therefore Alice and Bob can run any algorithm which gives an $(1+\eps)$ approximate matching to distinguish between the two cases of $\NGC_{n,k}$. 
	
	In our hard distribution for $\NGC_{n,k}$, we have $k = \Theta(\ln n)$. Thus for $\eps = \Theta\paren{\frac1{\ln n}}$, we know that the streaming algorithm requires $\Omega(n) = 2^{\Omega(1/\eps)}$ space.  
\end{proof}

